Scalable Peaceman-Rachford Splitting Method with Proximal Terms

Along with developing of Peaceman-Rachford Splittling Method (PRSM), many batch algorithms based on it have been studied very deeply. But almost no algorithm focused on the performance of stochastic version of PRSM. In this paper, we propose a new stochastic algorithm based on PRSM, prove its convergence rate in ergodic sense, and test its performance on both artificial and real data. We show that our proposed algorithm, Stochastic Scalable PRSM (SS-PRSM), enjoys the $O(1/K)$ convergence rate, which is the same as those newest stochastic algorithms that based on ADMM but faster than general Stochastic ADMM (which is $O(1/\sqrt{K})$). Our algorithm also owns wide flexibility, outperforms many state-of-the-art stochastic algorithms coming from ADMM, and has low memory cost in large-scale splitting optimization problems.

==> Alg4SCG.tex <==
\begin{algorithm}[H]
	\caption{SCG-SCPRSM (one step)}
	\label{SCG}
    \begin{algorithmic}[1]
\State Specify $\tau\in(0,1)$; $q_1\in(0,0.5)$; $q_2\in(q_1,1)$; $\epsilon$ close to 0;
\State Set $\tilde{\bx}_1=\bx_1^k$; $\bx_{1,0}=\tilde{\bx}_1$; $\tilde{\mu}=1$; $t=0$;
\State Set $\bs_0=-(G_{\beta}^k)'(\bx_{1,0})$; $\bh_0=\bs_0$;
\While{$\|\bs_t\|_2> \epsilon$}
\State Randomly draw $\xi_{k+1}$ from $\U\{1,n\}$;
%\State $\bs_t=-(G_{\beta}^k)'(\bx_{1,t},\xi_{k+1})$;
\State $\eta=1$; $v_h=1$; $v=0$; $\bp_h=\b0$; $\bp=\b0$;
\While{$v_h>v+q_1\eta\bh_t^T\bp$ $||$ $\bh_t^T\bp_h<q_2\bh_t^T\bp$} \Comment{Wolfe criterion}
\State $v_{h}=G_{\beta}^k(\bx_{1,t}+\eta\bh_t,\xi_{k+1})$; $\bp_{h}=(G_{\beta}^k)'(\bx_{1,t}+\eta\bh_t,\xi_{k+1})$;
\State $v=G_{\beta}^k(\bx_{1,t},\xi_{k+1})$; $\bp=(G_{\beta}^k)'(\bx_{1,t},\xi_{k+1})$;
\State $\eta=\tau\eta$;
\EndWhile
\State $t=t+1$;
\State $\bx_{1,t}=\bx_{1,t-1}+\frac{\eta}{\tau}\bh_{t-1}$;
\State $\bs_{t} = -(G_{\beta}^k)'(\bx_{1,t})$;
\State $\delta_{t}=\frac{\bs_{t}^T\bs_{t}}{\bs_{t-1}^T\bs_{t-1}}$; \Comment{Fletcher–Reeves formula ~\cite{fletcher1964function}}
\State $\bh_{t}=\bs_{t}+\delta_{t}\bh_{t-1}$;
\EndWhile
\State $\bx_1^{k+1}=\frac{1}{t+1}\sum_{i=0}^{t}\bx_{1,i}$.
  \end{algorithmic}
\end{algorithm}

==> useless.tex <==
have recently become a popular research topic.

SCAS-ADMM design for large-scale optimization problems with the same convergence rate of SA-ADMM, and does not need an extra memory to store the historic gradients on all samples decrease the storage cost.

From the convergence analysis of the above papers, it can be found that the proof of convergence rate of PRSM is much more difficult than ADMM.

Unlike the ADMM, there are few people doing the PRSM which has the better performance and there are little variants of the method. 
In this paper, we propose a couple of new variants of PRSM, called Scalable Stochastic Strictly Contractive Peaceman-Rachford Splitting Method (SS-PRSM) and Stochastic Conjugate Gradient Peaceman-Rachford Splitting Method (SCG-PRSM) for large-scale optimization problems. We get inspiration from the SCAS-ADMM to make the SS-PRSM algorithoms. The main features of our algorithms are outlined as follows:

\begin{enumerate}
	\item We combined the batch SPB-SCPRSM with the stochastic setting using the method of the stochastic variance reduced
	gradient (SVRG) to get the SS-PRSM. The computations of our algorithm for every update step are efficiently carried out.
	%\textit{Note}: we can get several algorithms like Stochastic ADMM and Stochastic SCPRSM by setting different semi-proximal terms and relaxation factors.
	\item SCG-PRSM is inspired by the conjugate gradient method. The Conjugate Gradient method only needs to use the first derivative information, and overcomes the shortcomings of the Gradient Descent method which may have slow convergence. Meanwhile the required storage capacity is small, and it has the advantage of high stability.
	\item We show that the convergence rate of the SS-PRSM algorithm is $O(1/t)$ as same as the batch ADMM, SCPRSM and SA-ADMM in the general convexity case. %When setting ($\alpha=0$), we get the SCAS-ADMM. So, we unify how to analyze the convergence rate of SCAS-ADMM. And
	And we show that the SCG-PRSM converge faster than the previous algorithms in several numerical experiments.
	%\item Our method does not require the storage of gradients, and thus is more easily applicable to complex problems such as some structured prediction problems and neural network learning.
\end{enumerate}

%We begin by presenting the background of splitting problem in Section~\ref{sec:background}. In Section~\ref{sec:algorithm},  we propose the iteration of our main algorithm (Stochastic SPB-SPRSM). The main results of convergence rate is provided in Section~\ref{sec:conv}. The experimental results on simulated and real datasets are presented in Section~\ref{sec:4}. Finally, we give conclusions as well as future possible work in Section~\ref{sec:summary}. Our proofs are included in the appendix.

